A Quantum Query Complexity Trichotomy for Regular Languages

We present a trichotomy theorem for the quantum query complexity of regular languages. Every regular language has quantum query complexity Theta(1), ~Theta(sqrt n), or Theta(n). The extreme uniformity of regular languages prevents them from taking any other asymptotic complexity. This is in contrast to even the context-free languages, which we show can have query complexity Theta(n^c) for all computable c in [1/2,1]. Our result implies an equivalent trichotomy for the approximate degree of regular languages, and a dichotomy---either Theta(1) or Theta(n)---for sensitivity, block sensitivity, certificate complexity, deterministic query complexity, and randomized query complexity. The heart of the classification theorem is an explicit quantum algorithm which decides membership in any star-free language in ~O(sqrt n) time. This well-studied family of the regular languages admits many interesting characterizations, for instance, as those languages expressible as sentences in first-order logic over the natural numbers with the less-than relation. Therefore, not only do the star-free languages capture functions such as OR, they can also express functions such as "there exist a pair of 2's such that everything between them is a 0." Thus, we view the algorithm for star-free languages as a nontrivial generalization of Grover's algorithm which extends the quantum quadratic speedup to a much wider range of string-processing algorithms than was previously known. We show a variety of applications---new quantum algorithms for dynamic constant-depth Boolean formulas, balanced parentheses nested constantly many levels deep, binary addition, a restricted word break problem, and path-discovery in narrow grids---all obtained as immediate consequences of our classification theorem.

==> sections/swamplands.tex <==
%!TEX root = ../reg-query.tex

\section{Dispensing with the trivial languages}
\label{sec:swamplands}

We now need to argue that are monoid characterizations are correct.  We first show that the query complexities of various regular languages can only fall into certain categories.  We then show that the syntactic monoid of those languages in those classes matches with the characterizations in Theorem~\ref{thm:monoid_characterizations}.  Let us start with the degenerate languages. 

\begin{proposition}
For fixed alphabet $\Sigma$, there are only four flat degenerate languages: $\varnothing$, $\Sigma^{*}$, $\{ \varepsilon \}$, or $\Sigma^+$.  Furthermore, if $L\subseteq \Sigma^{*}$ is a flat regular language and not one of those four, then $\approxdeg(L) \geq 1$.
\end{proposition}
\begin{proof}
First, we claim that the syntactic monoid of each language, $\varnothing$, $\Sigma^{*}$, $\{ \varepsilon \}$, or $\Sigma^+$, satisfies the monoid characterization of Theorem~\ref{thm:monoid_characterizations}.   This calculation is straightforward, and we leave it as an exercise.  

Let $L$ be a flat regular language, and let $\varphi$ be the homomorphism onto its syntactic monoid $M_L$ such that $L = \{ \varphi^{-1}(s) : s \in S \subseteq M_L \}$.  We wish to show that if $L$ is not one of $\varnothing$, $\Sigma^{*}$, $\{ \varepsilon \}$, or $\Sigma^+$, then its syntactic monoid is not degenerate; that is, there exist $x, y \in \Sigma^+$ such that $\varphi(x) \neq \varphi(y)$.  However, if $L$ is not one of $\varnothing$, $\Sigma^{*}$, $\{ \varepsilon \}$, or $\Sigma^+$, then there must exist $x,y \in \Sigma^+$ such that $x \in L$ but $y \not \in L$.  Since $L$ is the image $\varphi^{-1}(S)$, it must be that $\varphi(x) \in S$ but $\varphi(y) \not \in S$, so $\varphi(x) \neq \varphi(y)$.

Finally, we argue that $\approxdeg(L) \geq 1$ if $L$ is not one of the four degenerate languages.  First, if $L$ is not degenerate, there exists monoid elements $r \in M_L$ such that $r \not \in S$ and $\varphi^{-1}(r)$ contains a nonempty string; similarly, there exists $s \in S$ such that $\varphi^{-1}$ contains a nonempty string.   Since $L$ is flat, each set $\varphi^{-1}(r)$ and $\varphi^{-1}(s)$ contains strings of all positive lengths (see Definition~\ref{def:flat}).  Therefore, any polynomial approximating the membership function for $L$ cannot be constant.
\end{proof}


%\subsection{\texorpdfstring{$O(1)$}{O(1)}-complexity languages are trivial}

Finally, we need to argue that $O(1)$-complexity languages are trivial, otherwise there could be, e.g., nontrivial star-free languages with $O(1)$-complexity. By Theorem~\ref{thm:TODO}, if the deterministic query complexity of $L$ is $O(1)$, then so is sensitivity, certificate complexity, quantum query complexity, etc.  Therefore, for the purposes of the proof we will consider only deterministic query complexity. 

\begin{theorem}
Let $L$ be a flat regular language. If the deterministic query complexity of $L$ is constant, then $L$ is a trivial language. 
\end{theorem}
\begin{proof}
Recall that a deterministic query algorithm is a decision tree:  on input $x \in \Sigma^*$, the algorithm queries a particular index of the input and based on the value of the input at that index (one of finitely many possible choices), the algorithm either deduces the membership of $x$ in $L$ or decides to query a different index.  The process is repeated until the algorithm can decide membership.  The height of the decision tree is the deterministic query complexity of $L$.  In particular, if the deterministic query complexity of $L$ is constant, then the height of the decision tree is constant, which implies that the entire tree has constant size (since each node in the tree has constant fan-out).  That is, for any input $x \in \Sigma^n$, the deterministic algorithm queries a constant-size set of indices to determine membership.

Clearly, as $n$ increases, there will be large gaps between the indices which are queried.  Since $L$ is flat we have two important consequences: first, any nonempty string which is not queried can correspond to any non-identity element of the syntactic monoid; second, we may assume that any gap of nonzero size can be expanded or contracted to any nonzero size. It follows that we can arbitrarily change the set of queries made by deterministic algorithm, provided that we do not create or destroy any gaps. For example, queries at the start or end of the input string cannot be moved. 

Therefore, let us move all the queries as close to the start of the input as possible, maintaining $1$-symbol gaps where necessary. Since there are only constantly many total queries, there exists a deterministic algorithm which determines membership of $x$ by querying $c$ symbols from the start and end of $x$ for some constant $c$.  

Let $\varphi$ be the homomorphism onto its syntactic monoid $M_L$ such that $L = \{ \varphi^{-1}(s) : s \in S \subseteq M_L \}$.  
%Let $r, s, t \in M_L \backslash \{1\}$ be any non-identity elements of the syntactic monoid.  By the above, 
For $x \in \Sigma^*$ of length greater than $2c$, write $x = u w v$ such that $|u| = |v| = c$.  We have that membership of $x$ in $L$ is determined completely by prefix $u$ and suffix $v$.  

We claim that this implies that $\varphi(u w v) = \varphi(u w' v)$ for all $w \in \Sigma^*$.  For suppose that $\varphi(w) \neq \varphi(w')$.  By the definition of flatness and the syntactic congruence, there exists strings $a \in \Sigma^c$ and $b \in \Sigma^c$ such that $a w b \in L$ and $a w' b \not \in L$.  This contradicts the fact that membership in $L$ is determined by the prefix and suffix of length at most $c$.  In particular, this holds when $w' = \varepsilon$.


%By Theorem~\ref{thm:phiequivalence}, we can use constantly many applications of this algorithm to compute $\varphi(w)$, where $w$ is the input string. Moreover, the string is the same in each application of the algorithm, except for the first and last symbol. Therefore we can compute $\varphi(w)$ from a length $c$ prefix and suffix of $w$. 

%Say $\varphi$ maps the first $c$ symbols to $r \in M \backslash \{ 1 \}$, the last $c$ symbols to $t \in M \backslash \{ 1 \}$, and the middle symbols to $s \in M \backslash \{ 1 \}$. Notice that $r$, $s$, and $t$ can be arbitrary elements of $M \backslash \{ 1 \}$ because $L$ is flat. We have just argued that $\varphi(w) = rst$ is determined (by the deterministic algorithm) solely on the basis of $r$ and $t$. That is, $rst = rs't$ for all $r, s, s', t \in M \backslash \{ 1 \}$. Also note that since $w$ was arbitrary, every non-identity monoid element is of the form $rst$. 

Let us now show that the syntactic monoid satisfies the rectangular band property.  Let $x,y,z \in \Sigma^+$ be nonempty strings, and let $x',z'$ be strings of length $c$ such that $\varphi(x) = \varphi(x')$ and $\varphi(z) = \varphi(z')$.
%, we have $\varphi(x) = \varphi(xx)$ and $\varphi(xyz) = \varphi(xz)$rst = rt$ for all $r,s,t \in M \backslash \{ 1 \}$.
We have that 
$$
\varphi(xyz) = \varphi(x' y z') = \varphi (x' z') = \varphi(xz).
$$
% First, take $r$ and write it as $r = mpq$ for some $m,p,q \in M \backslash \{ 1 \}$. Then 
%$$
%rt = mpqt = mpqst = rst.
%$$
Finally, we show that $\varphi(\Sigma^+)$ is idempotent.  Let $x \in \Sigma^+$.  By flatness, we have that $\varphi(x) = \varphi(a w b)$ for strings $a, b \in \Sigma^c$.  Therefore, we have
$$
\varphi(x) = \varphi(a w b) = \varphi(a b) = \varphi(a b a b) = \varphi(xx),
$$
where the middle two equalities come from substituting $w = \varepsilon$ and $w = ba$, respectively.
\end{proof}













